Hyper Temporal Networks

Simple Temporal Networks (STNs) provide a powerful and general tool for representing conjunctions of maximum delay constraints over ordered pairs of temporal variables. In this paper we introduce Hyper Temporal Networks (HyTNs), a strict generalization of STNs, to overcome the limitation of considering only conjunctions of constraints but maintaining a practical efficiency in the consistency check of the instances. In a Hyper Temporal Network a single temporal hyperarc constraint may be defined as a set of two or more maximum delay constraints which is satisfied when at least one of these delay constraints is satisfied. HyTNs are meant as a light generalization of STNs offering an interesting compromise. On one side, there exist practical pseudo-polynomial time algorithms for checking consistency and computing feasible schedules for HyTNs. On the other side, HyTNs offer a more powerful model accommodating natural constraints that cannot be expressed by STNs like Trigger off exactly delta min before (after) the occurrence of the first (last) event in a set., which are used to represent synchronization events in some process aware information systems/workflow models proposed in the literature.

==> preamble.tex <==
\usepackage[utf8]{inputenc} %if you compile by pdflatex
%\usepackage{fixltx2e} %if you compile by pdflatex

%AMS MATH deve stare prima della dichiarazione font
\usepackage[cmex10]{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{pbox}
% \usepackage{mathptmx}%Required by SVJour3 Con mathptmx mancano i font bold per math
%Ho trovato la seguente impostazione equivalente
\usepackage[T1]{fontenc}
%\usepackage{newtxtext,newtxmath}
% \usepackage{flushend}%to equalize the last column
% \usepackage{balance}
\RequirePackage{latexsym}
\RequirePackage{array}
\RequirePackage{xspace}
\RequirePackage{cite}
%\usepackage[switch,columnwise]{lineno}
\usepackage{graphicx}
\usepackage[font=small]{caption}
\usepackage[caption=false]{subfig}%opzione necessari altrimenti lancia warning
\usepackage{paralist}

%For decimal alignment in tabular
\usepackage{dcolumn}
\newcolumntype{d}[1]{D{.}{.}{#1} }
%\newtheorem{example}{Example}
%\graphicspath{{./Figures/}}
%\interdisplaylinepenalty=2500%Required by the IEEEtran
%\setlength{\extrarowheight}{1pt}
%tikz
\usepackage{tikz}%Front end per PGF, package di disegno 
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.units}
%\pgfplotsset{compat=1.6}
\usetikzlibrary{calc,positioning,fit}%calc e positioning permettono il posizionamento avanzato
\usetikzlibrary{shapes,shapes.multipart,shapes.arrows}
\usetikzlibrary{decorations,decorations.pathmorphing,decorations.pathreplacing,decorations.markings,decorations.shapes}
\usetikzlibrary{arrows}%se si usano le frecce diverse
%sano le frecce diverse   
\usetikzlibrary{fit,backgrounds}
\usetikzlibrary{plotmarks}

\makeatletter
% code by Andrew Stacey: http://tex.stackexchange.com/a/27996/3954
%usage: \path [through point=(n2.east)] (n1) edge (n3);
\tikzset{
  through point/.style={
    to path={%
      \pgfextra{%
        \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
        \pgfmathsetmacro{\pt@sx}{\pgf@x * 0.03514598035}%
        \pgfmathsetmacro{\pt@sy}{\pgf@y * 0.03514598035}%
        \tikz@scan@one@point\pgfutil@firstofone#1\relax
        \pgfmathsetmacro{\pt@ax}{\pgf@x * 0.03514598035 - \pt@sx}%
        \pgfmathsetmacro{\pt@ay}{\pgf@y * 0.03514598035 - \pt@sy}%
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \pgfmathsetmacro{\pt@ex}{\pgf@x * 0.03514598035 - \pt@sx}%
        \pgfmathsetmacro{\pt@ey}{\pgf@y * 0.03514598035 - \pt@sy}%
        \pgfmathsetmacro{\pt@len}{\pt@ex * \pt@ex + \pt@ey * \pt@ey}%
        \pgfmathsetmacro{\pt@t}{(\pt@ax * \pt@ex + \pt@ay * \pt@ey)/\pt@len}%
        \pgfmathsetmacro{\pt@t}{(\pt@t > .5 ? 1 - \pt@t : \pt@t)}%
        \pgfmathsetmacro{\pt@h}{(\pt@ax * \pt@ey - \pt@ay * \pt@ex)/\pt@len}%
        \pgfmathsetmacro{\pt@y}{\pt@h/(3 * \pt@t * (1 - \pt@t))}%
      }
      (\tikztostart) .. controls +(\pt@t * \pt@ex + \pt@y * \pt@ey, \pt@t * \pt@ey - \pt@y * \pt@ex) and +(-\pt@t * \pt@ex + \pt@y * \pt@ey, -\pt@t * \pt@ey - \pt@y * \pt@ex) .. (\tikztotarget)
    }
  }
}
\makeatother

%\usetikzlibrary{decorations,decorations.pathmorphing}
%un po' di stili comuni!
\tikzstyle{node}=[circle,draw,inner sep=2pt,transform shape,minimum size=1.75em,minimum width=.75cm]
%%
%% Nota per le label dentro le activity
%% Si vuole che l'etichetta sia su più righe:
%% 1) nome attività
%% 2) durata (scritta più piccola perché solitamente più lunga)
%% Come è noto LaTeX non permette di variare l'interlinea all'interno di un paragrafo in modo semplice.
%% Se si dichiara <nome>\\\scriptsize <durata>, l'interlinea sarebbe per \normalsize con l'effetto che la
%% seconda riga è a interlinea per \normalsize mentre il font è più piccolo: spazio sprecato per nulla.
%% Consultando le diverse FAQ, ho dedotto che la cosa migliore è:
%% Dichiarare come font per il paragrafo il più piccolo 
%% mettere in un environment {} la prima riga con la sua dichiarazione di font più grande: {\small <nome>} 
%% Circa il valore da inserire come text width, NON usare em, altrimenti il risultato non risulterà centrato
\tikzstyle{task}=[draw,rectangle,inner sep=1.5pt,transform shape
                         ,font=\sffamily\scriptsize,text width=27pt%vedi nota sopra
                         ,text centered,minimum height=2em
%                          ,gray
%                          ,line width=1pt
                         ]
\newcommand{\TaskText}[2]{{#1}\\{#2}}%%a capo funziona perché task ha l'opzione text width
% %
\tikzstyle{connector}=[draw,diamond,shape aspect=1,inner sep=1pt,transform shape
                 ,font=\sffamily\scriptsize,text width=15pt%vedi nota sopra. 
                 ,text centered
%                  ,gray
                 ]

\newcommand{\AND}{\tikz[baseline,arrows=-] \draw[thick] (0,2ex) -- (4ex,2ex) (2ex,0) -- (2ex,4ex);}%$\boldsymbol{+}$}
\newcommand{\DIS}{\tikz[baseline,arrows=-] \draw[thick] (0,2ex) -- (4ex,2ex) 
		(2ex,0) -- node[text width=,minimum width=0,font=\sffamily\scriptsize,rectangle,inner sep=0,outer sep=1pt,right,pos=.2,transform shape] {D}
		(2ex,4ex);}% ricorda che quando si usa \DIS dentro il connettore, il nodo eredita lo stile tikz 'connector'. Sono quindi necessari dei reset. $\boldsymbol{+}$}
\newcommand{\sDIS}{\tikz[baseline,arrows=-,transform shape] \draw[thick] (0,.95ex) -- (1.9ex,.95ex)
 		(.95ex,0) -- node[text width=,minimum width=0,font=\sffamily\tiny,rectangle,inner sep=0,outer sep=1pt,right,scale=.8,pos=.17,transform
 		shape] {D} (.95ex,1.9ex);}% ricorda che quando si usa \DIS dentro il connettore, il nodo eredita lo stile tikz 'connector'. Sono quindi necessari dei reset.
		% $\boldsymbol{+}$}
\newcommand{\sAND}{\tikz[baseline,arrows=-,scale=1] \draw[thick] (0,.75ex) -- (1.5ex,.75ex) (.75ex,0) -- (.75ex,1.5ex);}%$\boldsymbol{+}$}
\newcommand{\OR}{\tikz[baseline,arrows=-] \draw[thick] (0,0) -- (2ex,2ex) (0,2ex) -- (2ex,0);}%\textbf{X}}
\newcommand{\CHECKERText}[2]{%
 {\begin{tikzpicture}[baseline,thick,->]
         \draw (0,0) .. controls +(0:.3) and +(0:.3) .. (-.1,.4);
         \draw (-.1,.4) .. controls +(180:.3) and +(180:.3) .. (0,0); 
 \end{tikzpicture}}\\\textit{#1}\\ {#2}%
}
\newcommand{\TOT}{\AND}
%\newcommand{\OR}{\tikz[baseline,arrows=-] \draw[very thick] (0,0) -- (1.5ex,1.5ex) (0,1.5ex) -- (1.5ex,0);}%\textbf{X}}
\newcommand{\ALT}{\OR}
\newcommand{\ANDText}[2]{{\small\AND #1}\\ {#2}}%%a capo funziona perch<E9> connector ha l'opzione text width
\newcommand{\ORText}[2]{{\small\OR #1}\\ {#2}}%%a capo funziona perch<E9> connector ha l'opzione text width
\newcommand{\TOTText}[2]{{\TOT #1}\\ {#2}}%%a capo funziona perch<E9> connector ha l'opzione text width
\newcommand{\DISText}[2]{{\small\DIS #1}\\ {#2}}%%a capo funziona perch<E9> connector ha l'opzione text width
\newcommand{\ALTText}[2]{{\small\ALT #1}\\ {#2}}%%a capo funziona perch<E9> connector ha l'opzione text width
\newcommand{\IFText}[2]{{\textit{#1}}\\ {#2}}

%
\tikzstyle{multiHead}=[dashed,transform shape]
\tikzstyle{multiTail}=[dotted,thick,transform shape]
\tikzstyle{StartCase}=[circle,draw,minimum size=.75cm,transform shape]
\tikzstyle{EndCase}=[circle,draw,ultra thick,minimum size=.75cm,transform shape]
\tikzstyle{smallLabel}=[font=\sffamily\scriptsize,inner sep=1pt,transform shape]
\tikzstyle{timeLabel}=[smallLabel,midway,transform shape]
\tikzstyle{minWidth}=[text width=.9cm]
\tikzstyle{info}=[rounded corners,fill=yellow,text width=1cm,text centered,inner sep=1pt]
\tikzstyle{infoLine}=[thin,decorate,decoration={snake,amplitude=.4mm, segment length=2mm, post length=1mm}]
\tikzstyle{edgeLabel}=[font=\tiny,sloped]
\tikzstyle{infoRow}=[rounded corners,fill=yellow,inner sep=1pt]
\tikzstyle{punto}=[circle,draw,fill=black,minimum size=2bp,inner sep=0pt,outer sep=0pt]
\tikzstyle{blackNode}=[fill=black!30]
% \tikzstyle{puntoLinea}=[dash pattern=on 1pt off 3pt on 4pt off 3pt,>=angle 60] 
% \tikzstyle{axes}=[]
\tikzstyle{crosses}=[decorate,decoration={name=crosses,segment length=2mm,post length=2mm}]
\tikzstyle{every picture}=[>=latex]
\tikzstyle{every label}=[inner sep=2pt]
%\tikzstyle{information text}=[rounded corners, fill=red!10,inner sep=1ex]


%%%%
%%% General macros
%%%%
% %e.g. e i.e. necessitano di un aggiustamento di spaziatura.
\newcommand{\A}{{\cal A}}
\newcommand{\C}{{\cal C}}
\newcommand{\F}{{\cal F}}
\newcommand{\GTNC}[1][]{\textsc{General-\TN-Consistency#1}\xspace}
\renewcommand{\H}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\HTNC}[1][]{\textsc{Head-\TN-Consistency#1}\xspace}
\newcommand{\MPGD}[1][]{\textsc{\MPG{-}Decision#1}\xspace}
\hyphenation{Con-sis-ten-cy}
\newcommand{\MPGE}[1][]{\textsc{\MPG-Energy#1}\xspace}
\newcommand{\MPGT}[1][]{\textsc{\MPG-Threshold#1}\xspace}
\newcommand{\MPGS}{\textsc{\MPG-Synthesis}\xspace}
\newcommand{\MPGV}{\textsc{\MPG-Values}\xspace}
\newcommand{\MPG}{MPG\xspace}
\newcommand{\p}{{\textsf{P}}}
\newcommand{\NP}{{\textsf{NP}}}
\newcommand{\N}{\mathbf{N}\xspace}
\newcommand{\Ord}{\ensuremath{O}}
\newcommand{\Otilde}{\tilde{\Ord}}
\newcommand{\PP}{{\cal P}}
\newcommand{\Ppol}{{\!P}}
\newcommand{\Q}{\mathbf{Q}\xspace}
\newcommand{\R}{\mathbf{R}\xspace}
\newcommand{\STN}{STN\xspace}
\renewcommand{\S}{{\cal S}}
\newcommand{\TNC}[1][]{\textsc{\TN-Consistency#1}\xspace}
\newcommand{\TN}{HyTN\xspace}
\newcommand{\TTNC}[1][]{\textsc{Tail-\TN-Consistency#1}\xspace}
\newcommand{\UP}{{\textsf{UP}}}
\newcommand{\W}{{\cal W}}
\newcommand{\Z}{\mathbf{Z}\xspace}
\newcommand{\coNP}{{\text{co-}\NP}}
\newcommand{\coUP}{{\text{co-}\UP}}
\newcommand{\delay}{{\ell}}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\etal}{et al.\xspace}
\newcommand{\flow}{{f}}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\sm}{\setminus}
\newcommand{\wrt}{with respect to\xspace}
\newcommand{\wt}[1]{\widetilde{#1}}


%%%Command \cupdot for Romeo's disjoint union operator
\makeatletter
\providecommand*{\cupdot}{%
  \mathbin{%
    \mathpalette\@cupdot{}%
  }%
}
\newcommand*{\@cupdot}[2]{%
  \ooalign{%
    $\m@th#1\cup$\cr
    \sbox0{$#1\cup$}%
    \dimen@=\ht0 %
    \sbox0{$\m@th#1\cdot$}%
    \advance\dimen@ by -\ht0 %
    \dimen@=.5\dimen@
    \hidewidth\raise\dimen@\box0\hidewidth
  }%
}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{corollary}[]{Corollary}
\newtheorem{lemma}[]{Lemma}
%\newtheorem{Fact}[]{Fact}
%\newtheorem{App}{Application}

\theoremstyle{definition}
\newtheorem{definition}{Definition}

\theoremstyle{remark}
\newtheorem{remark}{Remark}

\newcommand{\figwidth}{.9\columnwidth}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}


%algorithm
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\SetCommentSty{textsf}
\SetKwRepeat{DoWhile}{do}{while}
\SetAlFnt{\small} 
%In order to use algorithm inside a Figure in two columns,
% put the following commands before the algorithm in the text
%\begin{figure}[!t]
% \removelatexerror
 % \begin{algorithm}[H]
\makeatletter
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\makeatother

\usepackage[bookmarks=false,hyperindex=false,hyperfootnotes=false,hidelinks]{hyperref}
%\usepackage{url}


% \usepackage{soul}%for strikethrough \st
\usepackage[normalem]{ulem}% Ha il comando \sout che è molto meglio del comando \st del package soul. 
%ulem mette a disposizione anche \uline{}, \uuline{},\uwave{},\xout{}, \dashuline{}, \dotuline{}  
%todonotes deve stare per ultimo
\usepackage[textsize=small,prependcaption]{todonotes}
\setlength{\marginparwidth}{2cm}
% \newcommand\comment[1]{\todo[color=yellow,caption={comment}]{#1}}
\newcommand{\noteRob}[2][noinline]{\todo[#1,color=yellow,author=Roberto]{#2}\xspace}
\newcommand{\noteCar}[2][noinline]{\todo[#1,color=teal,author=Carlo]{#2}\xspace}
\newcommand{\noteRom}[2][noinline]{\todo[#1,color=red,author=Romeo]{#2}\xspace}
\newcommand{\insRob}[1]{{\color{blue}\protect#1}\xspace}
\newcommand{\insCar}[1]{{\color{teal}\protect#1}\xspace}
\newcommand{\insRom}[1]{{\color{red}\protect#1}\xspace}
\newcommand{\delRob}[1]{{\color{blue}\sout{\protect#1}}\xspace}
\newcommand{\delRom}[1]{{\color{red}\sout{\protect#1}}\xspace}
\newcommand{\delCar}[1]{{\color{teal}\sout{\protect#1}}\xspace}
\newcommand{\commentRob}[1]{\fcolorbox{orange}{orange}{#1}\xspace}


==> sectMaxMin.tex <==
In this section we study alternative formulations of \TN{s} and provide their characterization.

Recall that, in Section~\ref{sect:background}, we have introduced hypergraphs $H=(V, \A)$ 
whose hyperarcs $A\in\A$ had one single tail $t_A$ and possibly multiple heads $H_A$. 
We observe that we may have considered hyperarcs with one head and multiple tails as well. 
In this way, we may introduce a new family of hypergraphs which we dub MinMax-hypergraphs.

\begin{definition}
A \textit{MinMax-hypergraph} $H$ is a pair $(V,\A)$, 
	where $V$ is the set of nodes, and $\A$ is the set of \textit{hyperarcs}.
	Each hyperarc $A\in \A$ is either:
\begin{itemize}
	\item weighted arc, \ie $A=(t,h,w)$ for $t,h\in V$ and $w\in \R$, 
		where $t$ is called the \textit{tail} of $A$ and $h$ is called the \emph{head} of $A$;
	\item Min-hyperarc, \ie $A=(t_A, (H_A, w_A))$ has a distinguished node $t_A$, called the \textit{tail} of $A$,
		and a nonempty weighted set $(H_A, w_A)$, where $H_A\subseteq V\setminus\{t_A\}$
		contains the \textit{heads} of $A$, and each head $v\in H_A$ is associated with a \textit{weight} $w_A(v)\in\R$;
	\item Max-hyperarc, \ie $A=((T_A, w_A), h_A)$ has a distinguished node $h_A$, called the \textit{head} of $A$, 
		and a nonempty weighted set $(T_A,w_A)$, where $T_A\subseteq V\setminus\{h_A\}$
		contains the \textit{tails} of $A$, and each tail $v\in T_A$ is associated with a \textit{weight} $w_A(v)\in\R$.
\end{itemize}
Moreover, if $\A$ contains no Max-hyperarcs, we say that $H$ is a \textit{Min-hypergraph}, 
or simply a hypergraph as in Section~\ref{sect:problemFormulation};
whereas, if $\A$ contains no Min-hyperarcs, we say that $H$ is a \textit{Max-hypergraph}. 
\end{definition}

We introduce a corresponding notion of consistency in the following definition.

\begin{definition}[\MMTNC] A MaxMin-\TN \mbox{$H=(V,\A)$} is \emph{consistent}
              if it admits a \emph{feasible scheduling function},
             \ie if we can assign a real value $s(v)$ to each time-point $v$,
             such that each hyperarc $A\in\A$ is satisfied:
\begin{itemize}
\item if $A=(t,h,w)$ is a weighted arc, then, $s$ satisfies $A$ iff $s(h)-s(t)\leq w$; 
\item if $A=(t_A, (H_A, w_A))$ is a Min-hyperarc, then, $s$ satisfies $A$ iff
\[
   s(t_A) \geq \min_{v\in H_A} \{s(v) - w_A(v) \} \hspace{1cm} \forall A\in \A;
\]
\item if $A=((T_A, w_A), h_A)$ is a Max-hyperarc, then, $s$ satisfies $A$ iff 
\[
   s(h_A) \leq \max_{v\in T_A} \{s(v) + w_A(v) \}  \hspace{1cm} \forall A\in \A.
\]
\end{itemize}
\end{definition}

\begin{theorem} \MMTNC is \NP-Complete; 
even if input instances $(V, \A)$ are restriced to satisfy 
$w_A\in\{-1, 0, 1\}$ and $|H_A|, |T_A|\leq 2$
for every $A\in\A$.
\end{theorem}
\begin{proof} Any feasible scheduling can be verified in polynomial time, hence, \MMTNC lies in \NP.
To show that the problem is \NP-hard we show a linear reduction from 3-SAT. 
Let us consider a boolean 3-CNF formula with $n\geq 1$ variables and $m\geq 1$ clauses: 
\[\varphi(x_1, \ldots, x_n) = \bigwedge_{i=1}^m (\alpha_i \vee \beta_i \vee \gamma_i)\]
where $\C_i = (\alpha_i \vee \beta_i \vee \gamma_i)$ is the $i$-th clause of $\varphi$ 
and  each $\alpha_i,\beta_i,\gamma_i\in \{x_j, \neg x_j\mid 1\leq j\leq n\}$ is a positive or negative literal. 
We associate to $\varphi$ a MaxMin-\TN $H_{\varphi}=(V, \A)$ defined as follows:
\begin{itemize}
	\item $V=\{\textbf{0}, x_i, \neg x_i, \C_j \mid 1\leq i \leq n, 1\leq j\leq m\}$;
	\item $\A = \bigcup_{i=1}^n \text{Var}_i \cup \bigcup_{j=1}^m\text{Cla}_j$, where:
	\begin{itemize}
		\item $\text{Var}_i=\Big\{ 
			(\textbf{0}, x_i, 1), (x_i, \textbf{0}, 0), (\textbf{0}, \neg x_i, 1), (\neg x_i, \textbf{0}, 0), \\
			 (\{(x_i, -1), (\neg x_i, -1)\}, \textbf{0}),\\ 
			 (\textbf{0}, \{(x_i, 0), (\neg x_i, 0)\})\Big\}$. 
	\\ This defines the variable gadget for $x_i$. \\
	See Figure~\ref{FIG:Var_i} for an illustration; 
		\item $\text{Cla}_i=\Big\{(\textbf{0}, \C_i, 1), (\C_i, \textbf{0}, -1), \\
					(\{(\alpha_i, 0), (\beta_i, 0), (\gamma_i, 0)\}, \C_i)\Big | 
					\C_i = (\alpha_i \vee \beta_i \vee \gamma_i)\Big\}$ . 
	\\This defines the clause gadget for $\C_i$. \\
	See Figure~\ref{FIG:Cl_i} for an illustration.
	\end{itemize}
\end{itemize}
Notice that $|V|=1+2n+m=O(m+n)$ and $m_{\A}=8n+5m=O(m+n)$, hence, the transformation is indeed linearly bounded in time and space.
Moreover, notice that $\varphi$ is satisfiable if and only if $H_{\varphi}$ is consistent. 
In fact, any thruth assignment $\nu$ satisfying $\varphi$ can be  
translated into a feasible scheduling $s$ of $H_{\varphi}$ and vice-versa, 
\ie for every $1\leq i\leq n, 1\leq j\leq m$ we have 
$s(\textbf{0})=0; s(\C_j)=1; s(x_i)=\nu(x_i); 
s(\neg x_i)=0$ iff $\nu(x_i)=1$ and $s(\neg x_i)=1$ iff $\nu(x_i)=0$. 
\end{proof}

\begin{figure}[tb]
\centering
\begin{tikzpicture}[arrows=->,scale=1,node distance=3 and 3]
	\node[node, scale=1.2, label={below:$[0]$}, yshift=0ex] (zero) {$\textbf{0}$};
	\node[node, above right=of zero, xshift=0ex, yshift=0ex] (nX) {$\neg x_i$};
	\node[node, scale=1.2, above left=of zero, xshift=0ex] (X) {$x_i$};
 	%arcs
	%%%%%%% X's arcs %%%%%%
	\draw[] (zero) to [bend left=50] node[xshift=0ex, yshift=0ex,below] {$1$} (X); 
	\draw[] (X) to [bend left=50] node[above] {$0$} (zero);
	\draw[dashed, color=blue, thick] (zero) to [bend left=25] node[below] {$0$} (X);
	\draw[dashed, color=cyan, thick] (X) to [bend left=25] node[above] {$-1$} (zero);
	%%%%%%% nX's arcs %%%%%
	\draw[] (zero) to [bend left=50] node[xshift=-1ex, yshift=0ex,above] {$1$} (nX); 
	\draw[] (nX) to [bend left=50] node[xshift=1ex, yshift=0ex,below] {$0$} (zero); 	
	\draw[dashed, color=blue, thick] (zero) to [bend right=25] node[below] {$0$} (nX);
	\draw[dashed, color=cyan, thick] (nX) to [bend right=25] node[above] {$-1$} (zero);
\end{tikzpicture}
\caption{Gadget for a 3-SAT variable $x_i$.}
\label{FIG:Var_i}
\end{figure}

\begin{figure}[tb]
\centering
\begin{tikzpicture}[arrows=->,scale=0.5,node distance=4 and 2.5]
	\node[node, scale=1.3, label={above:$[1]$}] (one) {$\C_i$};
	\node[node, scale=1.3, below =of one, xshift=0ex, yshift=0ex] (beta) {$\beta_i$};
	\node[node, scale=1.3, left=of beta, xshift=-15ex] (alpha) {$\alpha_i$};
	\node[node, scale=1.3, right=of beta, xshift=15ex] (gamma) {$\gamma_i$};
 	\node[node, scale=1.3, label={below:$[0]$}, below=of beta, yshift=0ex] (zero) {$\textbf{0}$};
	 \node[xshift=12ex, left = of alpha] (fakeL) {};
 	 \node[xshift=-12ex, right = of gamma] (fakeR) {};
	%arcs
	%%%%%%% zero/one arcs %%%%%
	\draw[] (zero) to [bend left=55] node[xshift=-7ex, yshift=12ex,above] {$+1$} (fakeL.north); 
	\draw[] (fakeL) to [bend left=55] node[xshift=0ex, yshift=0ex,above] {} (one); 
	\draw[] (one) to [bend left=55] node[xshift=7ex, yshift=-15ex, above] {$-1$} (fakeR.south); 
	\draw[] (fakeR) to [bend left=55] node[xshift=0ex, yshift=0ex, above] {} (zero); 
	%%%%%%% alpha's arcs %%%%%%
	\draw[] (zero) to [bend left=50] node[xshift=0ex, yshift=0ex,below] {} (alpha); 
	\draw[] (alpha) to [bend left=20] node[above] {} (zero);
	\draw[dashed] (zero) to [bend left=25] node[below] {} (alpha);
	\draw[dashed] (alpha) to [bend left=5] node[above] {} (zero);
	\draw[dashed, color=blue, thick] (alpha) to [bend right=25] node[below] {$0$} (one.south);
	%%%%%%% beta's arcs %%%%%
	\draw[] (zero) to [bend left=50] node[xshift=-1ex, yshift=0ex,above] {} (beta); 
	\draw[] (beta) to [bend left=50] node[xshift=1ex, yshift=0ex,above] {} (zero); 	
	\draw[dashed] (zero) to [bend left=25] node[below, xshift=0ex] {} (beta);
	\draw[dashed] (beta) to [bend left=25] node[above, xshift=0ex, yshift=-3ex] {} (zero);
	\draw[dashed, color=blue, thick] (beta) to [] node[above, xshift=-1ex] {$0$} (one.south);	
	%%%%%%% gamma's arcs %%%%%%
	\draw[] (zero) to [bend right=50] node[xshift=0ex, yshift=0ex,below] {} (gamma); 
	\draw[] (gamma) to [bend right=20] node[above] {} (zero);
	\draw[dashed] (zero) to [bend right=25] node[below] {} (gamma);
	\draw[dashed] (gamma) to [bend right=5] node[above] {} (zero);
	\draw[dashed, color=blue, thick] (gamma) to [bend left=25] node[below] {$0$} (one.south);
\end{tikzpicture}
\caption{Gadget for a 3-SAT clause $\C_i = (\alpha_i \vee \beta_i \vee \gamma_i)$ 
where each $\alpha_i, \beta_i, \gamma_i$ is a positive or negative literal.}
\label{FIG:Cl_i}
\end{figure}

We conclude this section by observing that consistency problems for Min-hypergraphs and for Max-hypergraphs are inter-reducible, 
\ie we can solve consistency for any one of the two models in linear time whenever we  
have a procedure solving consistency for the other model.

\begin{theorem} \MaxTNC and \MinTNC are inter-reducible by means of $\log$-space, linear-time, local-replacement reductions.\end{theorem}
\begin{proof} We show the reduction from Max-hypergraphs to Min-hypergraphs; the other direction is symmetric.
Let $H=(V,\A)$ be a Max-hypergraph, we associate to $H$ a Min-hypergraph $H'=(V, \A')$ by reversing all Max-hyperarcs and by inverting the time-axis.
Formally, we define \[\A' = \{(h,t,w)\mid (t,h,w)\in A\}\cup\{(v, (S, w))\mid ((S, w), v)\in \A\}\] 
and we schedule $s_{H'}(v)=-s_{H}(v)$ for every $v \in V$.
Notice that $H$ is consistent if and only if $H'$ is consistent.
Indeed, for any hyperarc $A\in\A$ and provided that $A=((T_A, w_A), h_A)$ and $A'=(t_{A'}, (H_{A'}, w_{A'}))=(h_A, (T_A, w_A))$, 
we have $s_{H}(h_A)\leq \max_{v\in T_A} \{s(v) + w_A(v) \}$ iff 
$-s_{H}(h_A)\geq \min_{v\in T_A}\{-s_{H}(v) - w_A(v)\}$, \ie iff 
$s_{H'}(t_{A'})\geq \min_{v\in H_{A'}}\{s_{H'}(v)-w_{A'}(v)\}$. 
\end{proof}

In the remainder of this work we shall adopt Min-hypergraphs, 
already introduced in Section~\ref{sect:background} simply as hypergraphs, 
as the reference model.

